Towards Extending Noiseless Privacy -- Dependent Data and More Practical Approach

In 2011 Bhaskar et al. pointed out that in many cases one can ensure sufficient level of privacy without adding noise by utilizing adversarial uncertainty. Informally speaking, this observation comes from the fact that if at least a part of the data is randomized from the adversary's point of view, it can be effectively used for hiding other values. So far the approach to that idea in the literature was mostly purely asymptotic, which greatly limited its adaptation in real-life scenarios. In this paper we aim to make the concept of utilizing adversarial uncertainty not only an interesting theoretical idea, but rather a practically useful technique, complementary to differential privacy, which is the state-of-the-art definition of privacy. This requires non-asymptotic privacy guarantees, more realistic approach to the randomness inherently present in the data and to the adversary's knowledge. In our paper we extend the concept proposed by Bhaskar et al. and present some results for wider class of data. In particular we cover the data sets that are dependent. We also introduce rigorous adversarial model. Moreover, in contrast to most of previous papers in this field, we give detailed (non-asymptotic) results which is motivated by practical reasons. Note that it required a modified approach and more subtle mathematical tools, including Stein method which, to the best of our knowledge, was not used in privacy research before. Apart from that, we show how to combine adversarial uncertainty with differential privacy approach and explore synergy between them to enhance the privacy parameters already present in the data itself by adding small amount of noise.

==> helper.tex <==
helper


On one hand we want to collect usable data on the other hand protect users' privacy 

another protocol combining applied cryptography and differential techniques.

learn aggregate statistic without harming individual statistics 

periodic distributed stream aggregation model. An untrusted aggregator wishes to compute the sum of all 
users' values in each time period


aggregator obliviousness - aggregator only learns the noisy sum but no intermediate

failures of unknown subset of users 


Asymptotic analysis is misleading 

Authors present simulation results of performance 


Applications - learning distribution by approximation moments 

sensing and monitoring  public health and clinical research 

Shi NDSS 2011 

 

We believe that local trust  is convincing for various situation 
$O(\frac{(\log n)^{1.5}}{\epsilon}\sqrt{\frac{\kappa+1}{\gamma}}\sqrt{(\log\log n  + \log \frac{1}{\delta})\log\frac{1}{\eta} })$

